Comparisons of Experiments in Moral Hazard Problems

I use a novel approach to compare information in several classes of moral hazard problems: implementability, cost under risk neutrality and limited liability, and cost facing an agent with a general preference for money. Incentives in moral hazard problems are determined by the agent's state-dependent utility. Motivated by this observation, I define three nested geometric orders on information: the column space, the conic span, and the zonotope orders. Each order admits four equivalent characterizations: (i) inclusion of feasible state-dependent utility sets, (ii) dominance in the corresponding class of moral hazard problems, (iii) matrix factorizations, (iv) posterior belief distributions. In particular, the orders apply to both the classic and the flexible moral hazard problems, providing a unified framework to compare information.

==> body/app_5_general_agent_preference.tex <==

\section{Non-Separable Preferences \label{appsec:non-separable}}

This appendix relaxes the additive separability assumption on the
agent's preference. Results in Section \ref{sec:orders} continue
to hold under a more general form of additive-multiplicative payoff.
Most notably, this includes the case of exponential preferences. 

The only requirement is that the agent's risk attitude over money
does not depend on the action taken. That is, if the agent prefers
one lottery over money to another when taking some action, he ranks
them the same way when taking any other action. This is the risk independence
property introduced by \citet{keeney1973risk}. He shows that this
is equivalent to an additive-multiplicative representation: the agent's
payoff from taking action $\boldsymbol{\mu}$ and receiving payment
$t$ takes the form
\[
H(\boldsymbol{\mu})+K(\boldsymbol{\mu})u(t),
\]
where $u\in\mathcal{U}$ is the agent's utility from money, $H:\Delta\Omega\to\mathbb{R}\cup\left\{ -\infty\right\} $
is analogous to the cost function with negative infinity encoding
infeasibilities, and $K:\Delta\Omega\to\mathbb{R}_{++}$ is a multiplicative
weight on the utility from money. This is the functional form used
in \citet{grossman1983implicit}, though I impose weaker assumptions
on $H$ and $K$. Exponential preferences of the form $-\exp\left[-a\left(t-C(\boldsymbol{\mu}))\right)\right]$
are a special case with $H(\boldsymbol{\mu})=0$, $K(\boldsymbol{\mu})=\exp\left[aC(\boldsymbol{\mu})\right]$,
and $u(t)=-\exp\left(-at\right)$. The separable case in Section \ref{sec:MH-problems}
corresponds to $H(\boldsymbol{\mu})=-C(\boldsymbol{\mu})$ and $K(\boldsymbol{\mu})=1$. 

The additive-multiplicative form preserves the key property of the
baseline that the agent's problem is only parametrized by his state-dependent
utility. Given experiment $\mathcal{E}$ and contract $\boldsymbol{t}$,
the agent's expected payoff from action $\boldsymbol{\mu}$ is 
\[
H(\boldsymbol{\mu})+K(\boldsymbol{\mu})\boldsymbol{\mu}\cdot\boldsymbol{u},
\]
where $\boldsymbol{u}:=\mathcal{E}u(\boldsymbol{t})$ is the agent's
state-dependent utility. Both the incentive and participation constraints
depend on the contract $\boldsymbol{t}$ only through state-dependent
utility $\boldsymbol{u}$, given the target action $\boldsymbol{\mu}_{0}$. 

The orders in Section \ref{sec:orders} therefore carry through unchanged.
The sufficiency of the orders uses the same argument of larger set
of feasible state-dependent utilities. The necessity of the orders
uses the same constructive proof by setting $H(\boldsymbol{\mu})=-C(\boldsymbol{\mu})$
and $K(\boldsymbol{\mu})=1$. 

